Can We Learn Heuristics For Graphical Model Inference Using Reinforcement Learning?

Combinatorial optimization is frequently used in computer vision. For instance, in applications like semantic segmentation, human pose estimation and action recognition, programs are formulated for solving inference in Conditional Random Fields (CRFs) to produce a structured output that is consistent with visual features of the image. However, solving inference in CRFs is in general intractable, and approximation methods are computationally demanding and limited to unary, pairwise and hand-crafted forms of higher order potentials. In this paper, we show that we can learn program heuristics, i.e., policies, for solving inference in higher order CRFs for the task of semantic segmentation, using reinforcement learning. Our method solves inference tasks efficiently without imposing any constraints on the form of the potentials. We show compelling results on the Pascal VOC and MOTS datasets.

==> tab_results1.tex <==
\begin{table*}[!t]
\centering
{\scriptsize
\centering
\caption{\footnotesize{Performance results for minimizing energies with unary and pairwise potentials.  }}
\label{tab:Unary_Pairwise_Potential}
\setlength\tabcolsep{7pt}
\begin{tabular}{cccccccccccccc} \toprule
Nodes &    & \multicolumn{5}{c}{ Unary }  & \multicolumn{6}{c}{ Unary + Pairwise } \\ \cmidrule(lr){3-7} \cmidrule(lr){8-13}
            &                  &  $A^{*}$   & \multicolumn{2}{c}{\footnotesize{$r_{t}=-(E_{t}-E_{t-1}) $}} &  \multicolumn{2}{c}{ \footnotesize{$r_{t}=\pm1$}}  & $A^{*}$  &BP    & \multicolumn{2}{c}{\footnotesize{$r_{t}=-(E_{t}-E_{t-1}) $}} &  \multicolumn{2}{c}{ \footnotesize{$r_{t}=\pm1$}}
                                \\ \cmidrule(lr){4-5}  \cmidrule(lr){6-7}   \cmidrule(lr){10-11}  \cmidrule(lr){12-13} 
          
     &                      &              &    DQN    &   MCTS    &      DQN         &   MCTS             &               &                 &    DQN    &   MCTS     & DQN  & MCTS    \\  \midrule
25-50 &  Acc (sp)     &  \textbf{88.8}  &  87.3  &    86.9    &  \textbf{88.8}   &   \textbf{88.8}     &   88.9   & 88.9  & 83.5      &  87.6  &   88.8    & \textbf{88.9}    \\ 
      &  IoU (sp)    &  72.7   &  66.7  &   65.4    &      72.7          &  \textbf{72.8}  &     72.8  & 72.8   & 54.6     & 69.7   & 72.7       &  \textbf{72.8}    \\
      & Acc (p)      &  85.8  &  84.5   &   84.0    & \textbf{85.9}   &  85.8    &   85.9 & 85.9  & 81.0      &  84.8  & 85.9     & \textbf{85.9}    \\ 
      & IoU (p)      &   \textbf{58.6}   &  53.2   &  52.1     &     \textbf{58.6}  &   \textbf{58.6}   &  58.7   & 58.7    &  44.1     &  56.1  & 58.6     & \textbf{58.7}       \\ \midrule
 %    & Ratio          &   $-$            &   1.61            &   1.67    &   1.00         &  1.00   &     $-$       &    1.0   &     2.37     & 1.41     &   1.01  &  1.00   \\ \midrule
150-250 &  Acc(sp) &   86.3    &  86.4    &             85.8 &    86.3           &          86.4                  & 89.6    & 86.4    &  85.5      &  86.0      &     86.4       &  86.4 \\ 
       &  IoU (sp) &    63.2    &  63.4     &       56.3       &   63.2            &             63.4               & 69.2     &  63.4   &  52.4 &      56.7 &  63.3  & 63.3 \\
      & Acc (p)     &     85.6  &   85.7     &    85.0         &    85.6           &         85.7                   &  88.7     & 85.7     & 84.8 &       85.1 &  85.6 &  85.6 \\ 
      &     IoU (p)  &     60.1    &   60.3   &        53.8      & 59.7   &          60.3     &  65.2    &  60.4    &  49.7   &     54.5     &  60.2  & 60.2 \\\midrule
 %     & Ratio         &      $-$      &  1.07   &      1.52     &   1.03  &  1.00  &        $-$            &       1.9        &   2.1      &        &            &  \\  \midrule
350-500  & Acc (sp)  &  85.7   &     86.0   &      85.8     &   85.9    &              86.0              &  85.9   & 85.9  &  86.0    &     86.7     &    86.7   &  86.8\\ 
		&  IoU (sp) &  60.9   &    56.0   &      57.1       &   60.6      &         61.9                 & 61.9    & 61.9    &   61.7  &    62.9      &   62.9  &  63.0 \\
      & Acc (p)      & 85.0  &    85.4   &      85.3        &   85.3   &              85.5                & 85.4   &  85.4   &  85.4 &  86.2   &    86.2      &  86.2\\ 
      & IoU (p)       &  59.1   &     54.3   &     56.4      &  58.7     &           59.9                   &  59.9   & 59.9   &  59.7  &  60.8    &   60.8      & 60.9  \\\midrule
%      & Ratio          &  $-$     &              &               &            &                            &      $-$          &            &              &         &           &  \\  \midrule
\bottomrule
\end{tabular}}
\vspace{-0.25cm}
\end{table*}






==> tab_results2.tex <==

\begin{table*}[!t]
\centering
{\scriptsize
\centering
\caption{\footnotesize{Performance results for minimizing energies with higher order potentials. }}
\label{tab:HOC}
\setlength\tabcolsep{7pt}
\begin{tabular}{ccccccccccccc} \toprule
Nodes &    & \multicolumn{5}{c}{ Unary + Pairwise + HOP1 }  & \multicolumn{4}{c}{ Unary + Pairwise + HOP1 + HOP2} \\ \cmidrule(lr){3-7} \cmidrule(lr){8-11}
            &                  &  BP   & \multicolumn{2}{c}{\scriptsize{$r_{t}=-(E_{t}-E_{t-1}) $}} &  \multicolumn{2}{c}{ \scriptsize{$r_{t}=\pm1$}}   & \multicolumn{2}{c}{\scriptsize{$r_{t}=-(E_{t}-E_{t-1}) $}} &  \multicolumn{2}{c}{ \scriptsize{$r_{t}=\pm1$}}
                                \\ \cmidrule(lr){4-5}  \cmidrule(lr){6-7}   \cmidrule(lr){8-9}  \cmidrule(lr){10-11} 
          
     &                      &              &    DQN    &   MCTS    &      DQN     &   MCTS        &     DQN    &   MCTS     & DQN  & MCTS    \\  \midrule
25-50 &  Acc (sp)     &   91.6   & 89.8  &   90.4              & \textbf{91.7}    &        \textbf{91.7}        &   90.5         &   90.9       &     92.0      &       \textbf{92.1}      \\ 
      &  IoU (sp)    & 78.0       & 73.0 &   74.5      &   78.2    &   \textbf{78.4}          & 74.5      &     75.3            &    78.3   &       \textbf{78.6}         \\
      & Acc (p)      &  \textbf{87.9} & 86.4 &    86.7     &  \textbf{87.9}  &   \textbf{87.9}            &    86.9    &      87.3       & 88.0   &       \textbf{88.3}          \\ 
      & IoU (p)      & 61.2    &  57.1 &     57.7   &  \textbf{61.6}  &  \textbf{61.6} & 58.3   &        58.9 &  62.1    &        \textbf{62.2}       \\   \midrule
%     & Ratio          &    $-$    &       &              &       &          &  $-$   & $-$   &   $-$  & $-$  \\ \midrule
150-250 &  Acc(sp) &   89.7    &     88.2 &       89.0       &    89.7   &   \textbf{89. 8}      &   88.8  &         89.7     &  91.0    &    \textbf{ 91.6}        \\ 
       &  IoU (sp) &  69.4   &     63.7   &       66.7       &   \textbf{69.5}   &  \textbf{ 69.5}   &     66.8  &        67.5         & 70.0    &    \textbf{ 70.9}           \\
      & Acc (p)     &  88.8   &    87.4  &       88.2      &      \textbf{88.8}   &  \textbf{88.8}    &     88.1   &        88.8        &  89.2    &    \textbf{90.0}   \\ 
      &     IoU (p)  &   65.3   &   60.3   &      62.3        &   \textbf{65.4}   &      65.3   &     63.2  &        63.3         &  \textbf{66.0}   &   64.6   \\ \midrule
%      & Ratio         &                  &             &             &                         &                  &    $-$    &  $-$    &    $-$   &   $-$   \\  \midrule
350-500  & Acc (sp) &  89.2   &     88.8  &   89.2           &  89.3   &                 &   88.7   &                &  90.2     &      \\ 
		&  IoU (sp) & 68.0     &  62.5  &      64.7        &   67.9    &                 &  64.9  &                &   69.1  &     \\
      & Acc (p)       &  88.6   &    88.3 &        88.7      &   88.7    &                  & 88.0     &                  & 89.3               &      \\ 
      & IoU (p)       &   65.4   &  60.2   &     62.3         & 65.5  &                   &  62.6      &               &   66.1    &       \\ \midrule
%      & Ratio          &               &              &               &                      &                     &      $-$      &   $-$     &   $-$  &  $-$    \\  \midrule
\bottomrule
\end{tabular}}
\vspace{-0.25cm}
\end{table*}









